Weakly Supervised Video Representation Learning with Unaligned Text for Sequential Videos

Sequential video understanding, as an emerging video understanding task, has driven lots of researchers' attention because of its goal-oriented nature. This paper studies weakly supervised sequential video understanding where the accurate time-stamp level text-video alignment is not provided. We solve this task by borrowing ideas from CLIP. Specifically, we use a transformer to aggregate frame-level features for video representation and use a pre-trained text encoder to encode the texts corresponding to each action and the whole video, respectively. To model the correspondence between text and video, we propose a multiple granularity loss, where the video-paragraph contrastive loss enforces matching between the whole video and the complete script, and a fine-grained frame-sentence contrastive loss enforces the matching between each action and its description. As the frame-sentence correspondence is not available, we propose to use the fact that video actions happen sequentially in the temporal domain to generate pseudo frame-sentence correspondence and supervise the network training with the pseudo labels. Extensive experiments on video sequence verification and text-to-video matching show that our method outperforms baselines by a large margin, which validates the effectiveness of our proposed approach. Code is available at https://github.com/svip-lab/WeakSVR

==> tables/sim.tex <==
% Table generated by Excel2LaTeX from sheet 'tsm'
\begin{table*}[htbp]
    \centering
    
    \begin{tabular}{c|c|cc|c}
        \hline
        \textbf{Backbone}                                                                & \textbf{FZ Backbone}  & \textbf{ Dist} & \textbf{Fusion} & \textbf{CSV} \bigstrut \\
        \hline
        \multirow{4}[2]{*}{CLIP} &\ding{51} & L2                   & add            & 0.7742 \bigstrut[t]                                                                            \\
                                &\ding{51} & L2                   & concat         & 0.7822                                                                                         \\
                                &\ding{51} & Attn                 & add            & 0.7689                                                                                         \\
                                &\ding{51}  & Attn                 & concat         & 0.7771 \bigstrut[b]                                                                            \\
        \hline
    \end{tabular}%
    \caption{Add caption}
    \label{tab:sim}%
\end{table*}%

